Secure Incentivization for Decentralized Content Delivery

Prior research has proposed technical solutions to use peer-to-peer (P2P) content delivery to serve Internet video, showing that it can reduce costs to content providers. Yet, such methods have not become widespread except for a few niche instances. An important challenge is incentivization: what tangible benefits does P2P content delivery offer users who bring resources to the table? In this paper, we ask whether monetary incentives can help attract peers in P2P content delivery systems. We commissioned a professional survey of people around theUnited States to answer several relevant questions. We found that 51% of the 876 respondents--substantially larger than our expectations--answered "yes" to whether they would participate for suitable financial incentives. Encouraged by the results of the survey, we propose Gringotts, a system to structure incentives and securely incorporate P2P delivery into content delivery systems. Gringotts provides a novel Proof of Delivery mechanism that allows content providers to verify correct delivery of their files, and shows how to use cryptocurrency to pay peers while guarding against liars and Sybil attacks.

==> design-old.tex <==
\section{Design}


\subsection{Overview}

In \name, a file (or video) is stored in the form of chunks. Each chunk is placed on a number of ``peers'' participating in the service. When a ``client'' requests the ``Content Provider (CP)'' for a file, it replies with IP address of the peer it should contact for the first chunk (we will talk about routing and file placement in future sections). After the chunk is downloaded, client reports statistics (e.g., download speed) about the download back to CP. The client also verifies the integrity of the data by computing a hash specified by CP and reporting it back. CP informs the peer before a download begins, after the download is completed, the peer reports delivery to CP. This is done to detect if either peer or client are engaging is malicious behaviour by terminating the connection.

When both peer and client report a download for a particular chunk, the CP generates a self signed certificate, containing stats of download, time of generation and public key\footnote{This refers to public key associated with the cryptocurrency account of the peer} of peer. CP gives this certificate to the peer, which generates a ``Proof of Serving (PoS)'' using it private key, that contains this certificate.

Peer then submits the PoS to the blockchain for payment. The (CP) would have already placed a  ``Smart Contract'' for each file in the system, specifying that whoever produces a valid Proof of Serving for that file gets paid as per the smart contract. On receiving a valid PoS, the money is from CP's account to peer's account. The PoS is stored on the blockchain along with the associated transaction.

Including Peer ID in the certificate ensures that only the relevant peer can cash the certificate. Statistics of download can be used to provide differentiated payment based on quality of service (e.g., download speed) provided by the peer. Time of Day ensures that peer cashes the PoS in a short time frame after delivering the content. By self signing PoS, peer acknowledges service of content and that statistics of download reported by CP are correct.

The above process is repeated for every chunk. Figure \ref{fig:request_flow} shows overall flow for request of a file.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{images/request_flow.png}
    \caption{Flow of request for a file.}
    \label{fig:request_flow}
\end{figure}

\subsection{Thwarting Attacks}

Decentralization and incentivization bring in security challenges. In our threat model all the involved parties clients, peers and CPs can be malicious.  \pg{What more to write? Use blockchain for anomaly detection.}

\textbf{Collusion between Client and Peer}  If peer and clients collude, then peer and client can both lie about delivery of content, in the process making money without spending any resources. Anomaly detection strategies as used by ~\cite{rca} fail to detect such attacks. Our solution, prevents this attack by making the collusion economically infeasible. 

The CP randomizes the peers responsible for serving different chunks of the file when a request is made, making it difficult for the colluding client to contact the colluding peer. This is not enough, under the threat model where it takes 0 cost to create a new client, the malicious client can do the following. 1) Contact the CP for a file. 2) If the peer responsible for the first chunk is a colluding peer, then report back to CP acknowledging download without downloading anything. Colluding peer made money without spending any resources. 3) If the peer is not colluding, then terminate the connection and try again as a new client.

To avoid this, in \name{} the first chunk is downloaded from a secure/trusted node (e.g., another infrastructure CDN). This creates an overhead cost of downloading the first chunk in creating new clients. 

\textbf{Analysis}
For a particular file in a region, lets assume that the download cost for peers is $x$\$ per chunk, payment by CP is $y$\$ per chunk and upload cost for peers is $z$\$ per chunk in a ``region''. The fraction of malicious peers that owning chunks of the file is $m$ and $l$ is size of the file in chunks. 

In case of collusion, for a file download upto chunk $i$, the expected download cost for the client is, 

\begin{center}
    $Cost(i) = 1.x + (i-1).( m.0 + (1-m).x)$
\end{center}

The first chunk will be downloaded from a secure node (cost $x$). Out of the remaining $i-1$ chunks, if the requests within a region, are routed to peers with equal probability, then a fraction m will be downloaded with $0$ cost. The remaining chunk will be downloaded from honest peers with $(i-1).(1-m).x$ cost. Similarly payment to malicious peers for that download upto chunk $i$ in expectation is
\begin{center}
    $Payment(i) = (i-1).m.y$
\end{center}
The attack can be deemed economically infeasible if
\begin{center}
    $Payment(i) < Cost(i), \forall i \in \mathbb{N}$\\
    $y < x.(\frac{1}{m}-1)$
\end{center}

The constraint above puts a upper cap on payment. E.g., If payment for a file is twice that of download cost, then more than 33\% peers holding that file in the region, would have to collude together to make the attack economically feasible. In \name, the CP has to ensure ``randomization of peers'' for file placement as well and maintain a certain churn on file placement. If CP doesn't, then a small number of malicious peers can decide to hold a particular file in  a region, and achieve a high value of $m$ for that particular file. 

In out threat model, we also assume that creating peers have minimal costs. So, can a malicious entity without owning significant resources, create a large number of colluding peers, and carry out the attack. The answer is \textbf{No}, every colluding peer will still have to serve requests from honest clients, to do this each peer must contribute bandwidth resources. If a colluding peer drops these honest requests, then anomaly detection techniques can be used to identify such peers and quarantine them.

Note: This solution doesn't impose any extra load on a ``good'' client. Having said that it imposes the restriction of downloading the first chunk from a secure node, reducing the benefit of downloading the content using peers. The fraction of traffic that needs to served by a secure node is 1/$l$.

==> design_prateesh.tex <==
\section{Design}

In \name, the ``Content Provider''  creates a ``Smart Contract'' for each file to be served by the system. Smart Contract specifies what constitutes a ``Proof of Service (PoS)''. Whenever a ``peer'' serves content, it produces a PoS and submits it to the Blockchain. On receiving a valid PoS, money (cryptocurrency) is moved from content provider's account to peer's account. For posterity, a valid PoS is stored on the Blockchain along with the associated transaction. A file (or video) is stored in the form of chunks. Each chunk is placed on a number of peers participating in the service.


\subsection{Overview}

\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{images/request_flow.png}
    \caption{Flow of request for a file.}
    \label{fig:request_flow}
\end{figure}

Figure \ref{fig:request_flow} shows overall flow for request of a file. When a ``client'' requests the content provider for a file, it replies with an ``Initiating Certificate the content provider provides its IP address and the public key associated with its cryptocurrency account. IC also includes a unique ``Nonce'' or request ID for each request, and a default secure/trusted node (e.g., another CDN or content provider itself) to be contacted in case a peer is down. To avoid forging content provider signs IC with its private key.

Client downloads chunks sequentially from peers as indicated in the certificate, starting download for a chunk only after finishing the previous download. After each download the peer provides a PoS to the client. The client along with the IC, stores PoS for each chunk downloaded till now, forming a chain of PoS (PoSC) as shown in Figure ~\ref{fig:posc}. After every download, the client provides peer a hash of the PoSC and the nonce in IC. The peer generates a PoS by signing this hash using its private key. A PoSC is very similar to a Blockchain, every link in the chain can be verified by any third party. A unique nonce in IC couples with different peer list, insures that no to PoSC look the same. Both PoS and IC also contain time of day time stamps.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{images/PoSC.png}
    \caption{PoSC.}
    \label{fig:posc}
\end{figure}

In \name{}, the overhead on content provider in terms of client requests handled is similar to that of infrastructure based CDNs. In infrastructure based CDNs, when a client requests for a video, the request first goes to the content provider, which then provides a manifest file for the video. In \name, the content provider can include the certificate in the manifest file itself. The modified manifest file, also contains hash of each chunk, this allows client to verify data integrity.

\textbf{Can Blockchain handle such high transaction rates?} 
In the system described above, for every chunk delivery there will be a corresponding transaction, this might overwhelm the Blockchain. E.g, around 50,000 YouTube videos are watched every second, but a typical Blockchain like Etherum~\cite{ethereum} can only support 25 transaction per second. Moreover, the amount of each such transaction will be very small, making transaction costs high. 

A simple solution to this problem is to make payments probabilistic. To achieve this, a content provider can change the definition of a valid PoS, to say that a valid PoS in one which is divisible by a natural number $N$ pre-specified in the smart contract. This change reduces the number of transactions by a factor of $N$ so that we don't overwhelm the Blockchain. A peer now submits PoS only to Blockchain if it is divisible by $N$.

Since, not all PoSs are on the Blockchain, peers also submit the corresponding PoSC. Whenever a peer generates a valid PoS, it requests the PoSC from client. The Blockchain can verify the correctness of PoSC and of PoS, and accordingly move the money from content provider's account to Peer. Note that the overhead of sending the PoSC will occur only once in $N$ chunk download.

A very high $N$ means a high variation in the payment to a peer, on the other hand a low $N$ can overwhelm the Blockchain and can also lead to high transaction costs. Lets assume that we set the $N$ is such a way that an active peer gets paid 10 times per day, or 300 times a month on an average. The no of payouts in a month, will be Bernoulli distributed, with mean of 300 and relative standard deviation of only $1/\sqrt{300}$ or 5.7\%.
 
Ethereum supports ~2.2 million transactions per day. This implies that \name{} can support 220,000 active peers. Moreover, new Blockchains (e.g., Algorand~\cite{algorand}) already claim to support 100x the throughput, increasing active peers supported by \name{} to 22 million.

The payment strategy described over here ensures that if the download has happened correctly upto current chunk, then on producing a valid PoS peer will get paid. The payment is not dependent on what happens to the remaining chunks. 

\subsection{Detecting and Thwarting Attacks}

Decentralization and incentivization bring in security challenges. In our threat model all the concerned parties, clients, peers and content providers can be malicious. In this section, we consider financially motivated attacks and see how \name{} can detect and prevent them. There are two kinds of attacks possible, 1) Contert provider avoids paying peer, 2) peer makes money without spending resources. This leaves us with following attack scenarios i) Malicious peer, ii) Malicious content provider, iii) Collusion between client and content provider, and iv) Collusion between Client and peer. We don't consider attacks involving collusion of content provider and peer, as the money moves from content provider to peer, any attack cannot lead to financial gains.

\textbf{Malicious Peer} To get paid, a peer needs to generate a valid PoS, which requires PoSC provided by client. If a malicious peer doesn't serve the chunk, then the client simply won't supply the Hash of PoSC. Also since the peer only knows the Hash of PoSC, after serving the chunk, it cannot selectively choose the requests that will give a valid PoS. If the peer is down or doesn't provide PoS then the content is downloaded from the default.

\textbf{Malicious content provider} For each request content provider pick a new nonce. Since a content provider doesn't know the private key of the peer, it can't predict what the PoS will look like for a new nonce. content provider thus cannot pick a nonce to reduce the probability of a valid PoS to pay lesser. Content provider can however pick an old nonce that never lead to a valid PoS for a given peer list. To avoid this content provider has to pick monotonically increasing nonces for its requests. For each content provider, s peer is hosting a content for, it can remember the highest nonce seen still now.  If the peer sees a request containing smaller nonce, it can identify the content provider as being malicious and stop hosting content provider's content. 

\textbf{Collusion between client and content provider} In this setting the malicious client (in collusion with content provider) doesn't provide a PoSC, when the peer produces a valid PoS. When this happens, peers can simply quarantine the concerned content provider. The problem with this approach is that valid PoSs are generated rarely, a peer could have already spend substantial resources serving the content for malicious content provider. To remedy this we change step 6 of Figure~\ref{fig:request_flow}. Now, in step 6, if a peer produces a valid PoS or with a certain low probability $p$, it requests a PoSC before providing the PoS to client. Since client doesn't know how the PoS will look like, to avoid paying it would have avoid providing a PoSC on all such requests. If $p$ is higher than probability of payout per chunk download, then peer can identify the malicious behaviour without spending much resources. This solution also prevents attack where the malicious client provides peer a wrong hash or nonce in step 5 of Figure~\ref{fig:request_flow}.

An army of malicious clients can do a \textbf{Denial of Service(DoS)} attack on a particular content provider, by downloading files for that content provider but not following the protocol. The peers responsible for serving the files for that content provider, might end up quarantining it. To make a peer quarantine a content provider, the client will have to download content without following the protocol and be identified by the peer. Since peer requests client a PoSC with probability $p$ for every download, a client will have to download the chunk from peer, $O(1/p)$ times for peer to quarantine the content provider. As $p$ is low, carrying out a DoS attack of the aforementioned kind would consume significant resources.

\textbf{Collusion between Client and Peer (Sybil Attack)}  If peer and clients collude, then peer and client can both lie about delivery of content, in the process making money without spending any resources. Anomaly detection strategies as used by ~\cite{rca} fail to detect such attacks. Our solution, prevents this attack by making the collusion economically infeasible. 

The content provider randomizes the peers responsible for serving different chunks of the file when a request is made, making it difficult for the colluding client to contact the colluding peer. This is not enough, under the threat model where it takes 0 cost to create a new client, the malicious client can do the following. 1) Contact the content provider for a file. 2) If the peer responsible for the first chunk is a colluding peer, then generate PoS for the first chunk without actually downloading the file, then terminate the connection. Colluding peer made money without spending any resources. 3) If the peer is not colluding, then terminate the connection and try again as a new client.

To avoid this, in \name{} the first chunk is downloaded from a secure/trusted node (e.g., another infrastructure CDN). This creates an overhead cost of downloading the first chunk in creating new clients. 

\textbf{Analysis}
For a particular file, lets assume that the download cost for peers is $x$\$ per chunk, payment by content provider is $y$\$ per chunk and upload cost for peers is $z$\$ per chunk. The fraction of malicious peers that owning chunks of the file is $m$ and $l$ is size of the file in chunks. 

In case of collusion, for a file download upto chunk $i$, the expected download cost for the client is, 

\begin{center}
    $Cost(i) = 1.x + (i-1).( m.0 + (1-m).x)$
\end{center}

The first chunk will be downloaded from a secure node (cost $x$). Out of the remaining $i-1$ chunks, if the requests are routed to peers with equal probability, then a fraction m will be downloaded with $0$ cost. The remaining chunk will be downloaded from honest peers with $(i-1).(1-m).x$ cost. Similarly payment to malicious peers for that download upto chunk $i$ in expectation is
\begin{center}
    $Payment(i) = (i-1).m.y$
\end{center}
The attack can be deemed economically infeasible if
\begin{center}
    $Payment(i) < Cost(i), \forall i \in \mathbb{N}$\\
    $y < x.(\frac{1}{m}-1)$
\end{center}

The constraint above puts a upper cap on payment. E.g., If payment for a file is twice that of download cost, then more than 33\% peers holding that file, would have to collude together to make the attack economically feasible. In \name, the content provider has to ensure ``randomization of peers'' for file placement as well and maintain a certain churn on file placement. If content provider doesn't, then a small number of malicious peers can decide to hold a particular file, and achieve a high value of $m$ for that particular file. 

In out threat model, we also assume that creating peers have minimal costs. So, can a malicious entity without owning significant resources, create a large number of colluding peers, and carry out the attack. The answer is \textbf{No}, every colluding peer will still have to serve requests from honest clients, to do this each peer must contribute bandwidth resources. If a colluding peer drops these honest requests, then anomaly detection techniques can be used to identify such peers and quarantine them.

Note: This solution doesn't impose any extra load on a ``good'' client. Having said that it imposes the restriction of downloading the first chunk from a secure node, reducing the benefit of downloading the content using peers. The fraction of traffic that needs to served by a secure node is 1/$l$.


\subsection{Content Distribution/File Placement}

We propose creating a dynamic market place, where content providers and peers both agree on placing and serving a file. The goal of the content provider is to get desirable Quality of Service (QoS) (e.g., high download speed, low delay) for its files, while the goal of the peer is to make as much money as possible. 

To get good QoS for its files, a content provider should place its file on peers which have historically provided good QoS. To achieve this, the blockchain can be modified to record QoS metrics (as measured by the client) for  each  chunk whenever a transaction  happens. Now, a content provider can anticipate QoS provided by a potential peer by looking at QoS of transactions associated with that peer, and do file placement accordingly. 

Smart contracts can easily be modified, to make payment a function of QoS, time of day and file. Such a strategy can help content provider handle demands for a file that vary with time. E.g., A content provider could pay more for a file during times when demand is high (akin to surge pricing in uber). Similarly, content provider can also ensure specific QoS for different files. E.g., To avoid re-buffering of a video, content provider can say that peer will be paid only if the download speed is high enough to support minimum bit rate of video.

To reduce delays, a content provider should also take into account geographical location of peers and client, for file placement. If a file is popular in a particular region then the content provider should get more peers to serve the file in that region.

Peer's decision on whether it should host a particular file, will depend on it's own resources (e.g., bandwidth, storage) and the smart contract for file in question. The QoS provided by peer highly depends on number of requests routed to peer. To ensure a certain QoS, peer will also have to inform the content provider, the number of requests it can handle for a file.

An alternate design for content distribution is to use managed farms similar to Antfarm~\cite{antfarm}. Each content provider can act as a swarm co-ordinator for its own files, using statistics about its peers gathered from the blockchain.

\subsection{Routing}

In \name{}, during a request, content provider provides client, a randomized list of peers to be contacted for each chunk. In contrast to infrastructure based CDN, a content provider in ~\name{} incurs an extra overhead as a ``tracker'', keeping track of alive peers hosting its files. 

One solution to avoid  overheads is to do routing using Distributed Hash Table (DHT) based solution like Chord~\cite{chord} and Kademlia~\cite{kademlia}. However randomization in peer selection is challenging in DHTs, where malicious nodes can affect routing outcomes ~/cite{routingurdaneta2011survey}, exposing content providers to Sybil attacks. In addition to having security advantages, a partially centralized approach doesn't incur delays associated with peer discovery in DHT and can also be used to do more efficient routing in accordance with file placement.



%\textbf{Malicious Client} To avoid payment to a peer, a malicious client can provide wrong or no Hash of PoSC, Nonce in step 5 in Figure~\ref{fig:request_flow} or refuse to provide a PoSC when asked by a  peer. In such settings, a peer even after producing a valid PoS might not get paid, as it would fail to produce a correct PoSC. To remedy this we change step 6 of Figure~\ref{fig:request_flow}. Now, in step 6, if a peer produces a valid PoS or with a certain low probability $p$, it requests a PoSC before providing the PoS to client. Since client doesn't know how the PoS will look like, to avoid paying it would have avoid providing a PoSC on all such requests. If $p$ is much higher then probability of payout then peer can identify the malicious behaviour. The peer now doesn't provide the PoS, this implies that malicious peer will now have to redownload the file from a default node wasting bandwidth. If the process continues the peer can stop serving requests for the CP in question

==> intro.tex <==
\section{Introduction}

%Content delivery networks (CDNs) are widely used to improve the distribution of resources (e.g., images, videos) to end users. Large-scale CDNs, such as Akamai and CloudFlare, operate in geographically diverse locations, creating networks of proxy servers and datacenter machines that often span multiple ISPs. By directing user requests to CDN servers, content providers are able to seamlessly handle large demands for their resources without the associated infrastructure burdens.

% https://www.cisco.com/c/dam/en/us/solutions/collateral/service-provider/visual-networking-index-vni/complete-white-paper-c11-481360.pdf
%Recent years have seen dramatic increases in the bandwidth requirements on CDNs, with demands nearly doubling to 72 Petabytes (PB) per month since 2016. This surge in content delivery has been fueled by the steady increase in video consumption. CDNs are responsible for serving 70\% of globally streamed video, and recent reports suggest that video will account for 82\% of consumer Internet traffic by 2021, or 160 PB per month. Consequently, operational overheads for CDNs have increased, limiting CDNs from reducing costs for their customers, which can be prohibitively high for smaller content providers.

Content delivery networks (CDNs) like Akamai and CloudFlare are widely used to distribute resources (e.g., images, videos) to end users over their geographically distributed proxy servers. Recent years have seen dramatic increases in the bandwidth requirements on CDNs, with monthly demands nearly doubling to 72 Petabytes (PB) since 2016~\cite{ciscovideo}. This surge in content delivery has been fueled by the steady increase in video consumption. CDNs serve 70\% of globally streamed video, which is predicted to account for 82\% of consumer Internet traffic by 2021, or 160 PB per month~\cite{ciscovideo}. One would expect that these increases in bandwidth consumption would drive prices down for content providers. Yet CDN prices have remained relatively fixed~\cite{cdntrends}, and continue to be prohibitive for small organizations.

A promising approach to lower CDN prices, and the corresponding barrier of use, is to reduce bandwidth serving costs by leveraging cheaper Internet resources. Specifically, CDN networks can be augmented or replaced with resources supplied by autonomous individuals. For example, individuals can contribute unused bandwidth in their Internet plans to serve content on behalf of content providers. By serving content using bandwidth and storage resources that would otherwise be wasted, such systems are able to significantly reduce costs for all entities in the content distribution ecosystem.

Numerous academic and industrial systems have attempted to deploy content delivery platforms that leverage resources of individuals, both as supplements to traditional CDN infrastructure (hybrid CDNs)~\cite{netsessions,livesky}, or standalone, decentralized P2P systems~\cite{peer5,dandelion}. However, these approaches have provided limited benefits, largely due to lack of adoption with peers~\cite{p2psurvey}. For example, Akamai's NetSessions has witnessed adoption rates of only 30\%~\cite{netsessions}. Such lack of adoption not only increases service latency, as peers are unlikely to be in close proximity, but also limits bandwidth cost savings, since most content ends up being served from the original CDN infrastructure.

A natural solution to bolster adoption is to \textit{incentivize} individuals to contribute their resources to the service. Akin to how people participated in torrents to acquire files that were not available on the Internet, individuals need to benefit from serving files on behalf of content providers. Past incentivization strategies~\cite{dandelion,bittyrant,antfarm} in P2P file sharing systems employ ``tit-for-tat'' policies, which enable users of the service to contribute resources. For example, a common policy with such schemes is to force a user to serve X bytes before they can download Y bytes. However, these approaches only incentivize participants of the service, inherently limiting adoption. To make matters worse, not all service participants have resources to contribute, e.g., mobile clients with cellular data plans. Additionally, while past approaches do tackle certain challenges like ``free-loader'' issues, they cannot be applied directly to CDN-like settings which exhibit Byzantine behavior and are vulnerable to Sybil attacks (since collusion can result in a net gain for a party).

We believe that several recent trends motivate revisiting this challenge: increases in uplink bandwidth speeds~\cite{!!!}, and improvements in decentralized, cryptographically-secure transaction protocols. In this paper, we propose Marlin, a secure incentivization strategy that leverages these two trends, and increases adoption by decoupling resource contributions from service participation. With Marlin, people can independently become resource contributors (or ``peers'') and/or content consumers (or ``clients''). Our user study confirms that people are willing to contribute their unused resources if there are monetary incentives involved. However, applying this strategy to decentralized content delivery environments poses numerous challenges.

Marlin overcomes these challenges using several novel techniques. First, Marlin leverages Blockchains to enforce smart contracts in a way that securely provides and verifies monetary incentives to peers, without requiring any trusted parties. Second, Marlin includes new file sharing protocols that can prevent Sybil attacks by making them financially infeasible, without increasing overheads for properly functioning clients.\footnote{Note that this technique can be easily extended to hybrid or peer-assisted designs.} Existing routing and file placement strategies can be applied to Marlin. However, Marlin's third novel feature is that its incentivization approach also opens the door to new peering relationship protocols. For example, Marlin introduces \textit{dynamic peering contracts}, which enable content providers to dynamically adjust payment values based on demand, e.g., contracts whose price reflects current demand (akin to surge pricing with Uber).

We will outline each of the techniques described above, and explain the guarantees they provide with respect to security, reliability, and performance. Motivated by results from our 700-person user study, we will then outline the goals and requirements that people have with respect to participating in this service. Our user study results, coupled with the steady increases in user bandwidth~\cite{speedtest} and storage~\cite{!!!}, promote re-exploring the rich space of leveraging user resources for content delivery. We will conclude by discussing future directions that must be explored to realize this vision, as well as numerous other domains in which we believe secure, decentralized incentivization will be applicable.

==> intro3.tex <==
\section{Introduction}
\label{s:intro}

Video streams constitute over 70\% of global Internet traffic~\cite{ciscovideo,sandvine}. Most video is delivered to users today via Content Distribution Networks (CDNs) like Akamai and CloudFlare. Although CDN demand has nearly doubled since 2016~\cite{ciscovideo}, they are too expensive for many content providers~\cite{cdntrends}.

To combat these high prices, there have been many proposals to have peers cache and stream videos to each other, either as supplements to existing CDNs~\cite{netsessions,iqiyi,livesky}, or as decentralized P2P systems~\cite{peer5,dandelion}. For example, peers within an Internet Service Provider (ISP) in a city could stream videos directly to one another, avoiding expensive Internet paths. By serving content using bandwidth and storage resources that would otherwise go unused, such systems could significantly reduce costs for content providers and CDN operators.

%second paragraph similar to what we have but shorter. To combat this issue, researchers have proposed using peers to cache and stream videos to each other to save expensive wide-area bandwidth. For example, if you have CP and multiple users within Verizon FIOS network in Massachusetts, then they could stream data to each other directly, avoiding expensive long-haul paths. Have citations (9,8,7,4). 


These proposals have not seen significant adoption in practice because of a lack of significant participation~\cite{p2psurvey,netsessions}. Even forms of incentivization like virtual tokens and in-service perks (e.g., traffic prioritization) have failed to attract enough peers~\cite{dandelion, antfarm,bittyrant}. We believe that the steady increases in uplink bandwidth and storage capacity on laptops~\cite{speedtest} motivate revisiting P2P content delivery, but with a focus on secure payments as an incentive mechanism. %\ma{cryptographically-secure transaction protocols comes out of nowhere. Perhaps something like: '... as well as the development of decentralized, cryptographically-secure transaction protocols for providing monetary incentives...'}

%In this paper, we ask whether monetary incentives can address the adoption problem. 

We ask two questions. First, would users be willing to participate in such a system if they were incentivized with monetary payments? To answer this, we performed the first (to the best of our knowledge) large-scale user study aimed at understanding the requirements and concerns with respect to participation in P2P file sharing systems (\S\ref{s:userstudy}). Our key finding is that 51\% of the 876 users would participate, and those who would not participate were primarily concerned with device security, content liability issues, and impacts on device performance.

%Our key findings are that 1) 51\% of users would participate, 2) of those who would participate, 70\% expect to earn no more than 50\% of their monthly Internet bill, and 3) 27\% are willing to accept cryptocurrency payments (40\% reported ``maybe''), and 4) . To the best of our knowledge, we are the first to publish a study about user participation in decentralized file sharing systems.


% TODO: say that one approach for payment is to go through CP or CDN in a centralized way. However, this has two challenges: high transactional costs and trust CP is weird since they have different goals than peers (don't want to pay). So, this motivates decentralized approach. However, performing decentralized payments is challenging as no entity can be trusted. Our solution is novel method using blockchains to enforce smart contracts between peers an content providers. We limit overheads on the blockchain by..
%note that user study says people OK with cryptocurrency


Second, how can payments be done securely? One approach is to use a central party to regulate every payment transaction. 

but this suffers from two issues: 1) the per-transaction costs of identifying who to pay (and how much) are expensive, and 2) a single trusted entity can cheat the system since parties have conflicting goals (e.g., content providers want to minimize cost, while peers want to maximize payments). These challenges motivate a \textit{decentralized} payment network. However, secure payments in decentralized scenarios are challenging, as no party can be relied upon to  fully verify transactions. Our contribution is a novel decentralized payment method which employs Blockchains to enforce Smart Contracts between peers and content providers (\S\ref{s:design}). Our approach uses probabilistic payments to limit transaction overheads on the Blockchain. We believe that this approach is practical since our user study revealed that 27\% of users were willing to accept cryptocurrency payments, with 40\% noting ``maybe'' due to lack of familiarity.


%A primary challenge is that the transactional costs of identifying who to pay (and how much) is expensive, motivating a decentralized payment network. However, decentralized approaches are challenging in scenarios where no parties can be trusted. Our contribution is a novel method which employs Blockchains to enforce smart contracts between peers and content providers, without requiring any central or trusted party. Contract provider issues a smart contract for every file to be served, peers serving content for a CP produce a Proof of Service (PoS). Peers get paid on a presenting a valid PoS (as specified in the smart contract), the money then moves from content provider's account to  peer's.




%Second, how can monetary incentivization and payments be done securely? A primary challenge is that the transactional costs of identifying who to pay (and how much) is expensive, motivating a decentralized payment network. However, decentralized approaches are challenging in scenarios where no parties can be trusted. Our contribution is a novel method which employs Blockchains to enforce smart contracts between peers and content providers, without requiring any central or trusted party. Contract provider issues a smart contract for every file to be served, peers serving content for a CP produce a Proof of Service (PoS). Peers get paid on a presenting a valid PoS (as specified in the smart contract), the money then moves from content provider's account to  peer's.

%Third, once peers are incentivized to participate, how can we verify that they served the content they claim to have served, without trusting any one party?

Third, even with a decentralized payment system, how can we verify that peers served the content that they claim to have served? We present a lightweight solution in which content providers send clients an unforgeable certificate at the beginning of each file download, listing the peers to contact for each of the file's chunks. Each time a chunk is served, the corresponding peer provides a ``Proof of Delivery'' (PoD) to the client, who merges this with the initial certificate to generate a PoD chain. Thus, generating a valid PoD chain requires coordination between content providers, clients, and peers, each of whom have different goals. PoD chains are later stored on the Blockchain for distributed verification. We show that PoD chains are sufficient to prevent common attacks to decentralized file sharing architectures such as Sybil attacks (\S\ref{s:design}).
% TODO: in last sentence, add 'incentivization'

\ma{Do we need to discuss three challenges/contributions? I think there are two contributions: (1) the user study, (2) and the decentralized system for secure monetary incentivization. For (2), motivate decentralization and blockchain quickly, and then talk about the technical challenges in the content delivery setting: high load on the blockchain, verifying content delivery, Sybil attacks, etc. Importantly, we should focus on aspects of decentralized payments that are unique to content delivery. This sentence, for example, seems overly general: 'However, secure payments in decentralized scenarios are challenging, as no party can be relied upon to  fully verify transactions.'}

%Third, once peers are incentivized to participate, how can we verify that they did the work they are claiming to have done? How can we prove that they actually served content to clients, without trusting reports from any one party? 

%enforces peering relationships by specifying a list of peers to contact for donwloading each chunk of the file. Whenever a chunk is served, the peer provides the client a PoS, the client along with IC chains them to form a PoS Chain (PoSC) which can be verified by any third party. Generating a valid PoSC requires co-ordination between client, peer and the content provider, ensuring that work was actually down. PoS are later stored on the Blockchain, which acts as a secure log that supports distributed verification. Finally, our solution also includes transaction protocols to prevent against Sybil attacks.

%third paragraph: would such systems be adopted? this is important question because netsessions had only 30\% adoption rate. In this paper, we ask whether payments address this problem. We hit 3 challenges:
%- would users be willing to participate in this system (does incentivization with money work)? we are the first to publish user study about whether users are willing to participate for payment. here are some other high level results...
%- how do you do secure incentivization and payments in this system? challenge is transactional cost can be quite high so keeping track of who to pay with many users (and how much) is expensive, so payment network needs to be decentralized; however, decentralized settings where parties cannot be trusted poses challenges --> our contribution is that we propose method using blockchain/smart contracts
%- how do you verify that people did the work they are claiming to have done (validate people did the right thing, and authenticate their behavior)? we do that with certificates, sybil prevention techniques...
